InteractE: Improving Convolution-based Knowledge Graph Embeddings by Increasing Feature Interactions

Most existing knowledge graphs suffer from incompleteness, which can be alleviated by inferring missing links based on known facts. One popular way to accomplish this is to generate low-dimensional embeddings of entities and relations, and use these to make inferences. ConvE, a recently proposed approach, applies convolutional filters on 2D reshapings of entity and relation embeddings in order to capture rich interactions between their components. However, the number of interactions that ConvE can capture is limited. In this paper, we analyze how increasing the number of these interactions affects link prediction performance, and utilize our observations to propose InteractE. InteractE is based on three key ideas -- feature permutation, a novel feature reshaping, and circular convolution. Through extensive experiments, we find that InteractE outperforms state-of-the-art convolutional link prediction baselines on FB15k-237. Further, InteractE achieves an MRR score that is 9%, 7.5%, and 23% better than ConvE on the FB15k-237, WN18RR and YAGO3-10 datasets respectively. The results validate our central hypothesis -- that increasing feature interaction is beneficial to link prediction performance. We make the source code of InteractE available to encourage reproducible research.

==> sections/gcn_back.tex <==

%In this section, we give a brief overview of Graph Convolutional Networks (GCNs) \cite{Bruna2013,Defferrard2016,Kipf2016} for undirected graphs and its extension to directed labeled graphs.
%
%\subsection{GCN on Undirected Graph}
%Given a graph $\m{G} = (\m{V}, \m{E}, \m{X})$, where $\m{V}$ denotes the set of vertices, $\m{E}$ is the set of edges and $\m{X} \in \mathbb{R}^{|\m{V}| \times d} $ represents the input features of each node. The node representation obtained from a Graph Convolutional Network is defined as
%\[ \bm{H} = f((\bm{\tilde{D}}^{-\frac{1}{2}} (\bm{A}+ \bm{I}) \bm{\tilde{D}}^{-\frac{1}{2}})\m{X} \bm{W}) . \]
%Here, $\bm{A}$ denotes the adjacency matrix and $\bm{\tilde{D}}$ is defined as $\bm{\tilde{D}}_{ii} = \sum_{j}(\bm{A}+\bm{I})_{ij}$. The model parameter is denoted by $\bm{W}$ and $f$ is any activation function used\footnote{In this paper, we use ReLU, $f(x)=\mathrm{max}(0, x).$}. In terms of an individual node $v$, the above equation can be reformulated as
%\begin{equation}
%\bm{h}_{v} = f \left(\sum_{u \in \mathcal{N}(v)}\bm{W} \bm{x}_{u} + \bm{b} \right) ,~~~\forall v \in \mathcal{V}.
%\label{eqn:gcn_undirected}
%\end{equation}
%where, $\bm{h}_{v}$ is the obtained representation of the node $v$, $\bm{b} \in \mathbb{R} ^d$ denotes bias and $\m{N}(v)$ is the set of neighbors of $v$ in graph $\m{G}$. GCN representation $\bm{h}_{v}$ encodes immediate neighborhood of each node in the graph. For capturing multi-hop dependencies, several GCN layers can stacked one on the top of another. The representation of node $v$ obtained after $k$ layers of GCN is given as
%\begin{equation}
%\bm{h}^{k+1}_{v} = f\left(\sum_{u \in \m{N}(v)}\left(\bm{W}^{k} \bm{h}^{k}_{u} + \bm{b}^{k}\right)\right), \forall v \in \m{V} .
%\label{eqn:gcn_undir_main}
%\end{equation}
%where, $\bm{W}^{k}$ and $\bm{b}^{k}$ are the layer specific model parameters. 
%
%\subsection{GCN on Labeled Directed Graph}
%For a directed labeled graph $\m{G} = (\m{V}, \m{E}, \m{X})$, where each edge between two nodes $u$ to $v$ has a label $l_{uv}$. The GCN formulation as devised by \citet{gcn_srl} is based on the assumption that information in a directed edge flows along both the direction. Hence, for each edge $(u,v,l_{uv}) \in \m{E}$, an inverse edge $(v,u,l_{uv}^{-1})$ is included in $\m{G}$, generating an extended edge set $\m{E'}$. The representation obtained for a node $v$ after $k$ layers of directed GCN is given as 
%\begin{equation}
%\bm{h}^{k+1}_{v} = f\left(\sum_{u \in \m{N}(v)}\left(\bm{W}_{l_{uv}}^{k} \bm{h}^{k}_{u} + \bm{b}_{l_{uv}}^{k}\right)\right), \forall v \in \m{V} .
%\label{eqn:gcn_dir_main}
%\end{equation}
%
%Here, $\bm{W}_{l_{uv}}^{k}, \bm{b}_{l_{uv}}^{k}$ denote the direction and label specific parameter of the model. For suppressing erroneous edges in the graph, \citet{gcn_srl} also propose edge-wise gating which computes a score for each during GCN aggregation. The score is computed independently for each layer and is defined as
%\begin{equation}
%\label{eqn:edge_gating}
%g^{k}_{uv} = \sigma \left( h^{k}_u \cdot \hat{w}^{k}_{l_{uv}}  + \hat{b}^{k}_{l_{uv}} \right),
%\end{equation}
%where, $\hat{w}^{k}_{l_{uv}} \in \mathbb{R}^d$ and $\hat{b}^{k}_{l_{uv}} \in \mathbb{R}$ are learnable parameters and $\sigma(\cdot)$ denotes the sigmoid function. The above formulation leads to overparameterization when the number of relations in a Graph are large, for instance in Knowledge Graphs. To address this issue, \citet{r_gcn} propose basis and block-diagonal decomposition of $\bm{W}_{l_{uv}}^{k}$ for regularizing GCNs.
